The 15-Minute City Quantified Using Mobility Data

Americans travel 7 to 9 miles on average for shopping and recreational activities, which is far longer than the 15-minute (walking) city advocated by ecologically-oriented urban planners. This paper provides a comprehensive analysis of local trip behavior in US cities using GPS data on individual trips from 40 million mobile devices. We define local usage as the share of trips made within 15-minutes walking distance from home, and find that the median US city resident makes only 12% of their daily trips within such a short distance. We find that differences in access to local services can explain eighty percent of the variation in 15-minute usage across metropolitan areas and 74 percent of the variation in usage within metropolitan areas. Differences in historic zoning permissiveness within New York suggest a causal link between access and usage, and that less restrictive zoning rules, such as permitting more mixed-use development, would lead to shorter travel times. Finally, we document a strong correlation between local usage and experienced segregation for poorer, but not richer, urbanites, which suggests that 15-minute cities may also exacerbate the social isolation of marginalized communities.

==> 15 Minutes-4/tables/access_metrics_correlations.tex <==
\begin{table}[H]
    \centering
    \caption{Comparison of local access metrics}
    \label{access metrics corr}
\resizebox{\textwidth}{!}{\begin{tabular}{lrrrrrrrr}
\toprule
 & &\multicolumn{7}{c}{Counts of Amenities within a 15-minute walk (CBG-level)} \\
\cmidrule(l{3pt}r{3pt}){3-9}
 & Equal-Weighted Access & All & Healthcare & Restaurants & Services & Groceries & Religious & Arts and Culture\\
 & (1) & (2) & (3) &(4) & (5) &(6) & (7) & (8)\\
\midrule
Correlation with Access & 0.98 & 0.51 & 0.37 & 0.45 & 0.52 & 0.60 & 0.59 & 0.30 \\
\bottomrule
\end{tabular}}
\begin{minipage}{1\linewidth}
\scriptsize \textsl{Notes.---} The table shows neighborhood level correlations between different measures of local access to services and amenities. Column one provides the correlation between our main access index and an alternative measure of access, where the scores associated with the number of amenities in each category are added with equal weights. Columns 2--8 provide correlations between our baseline measure and counts of the number of each type of amenity within a 15-minute walkshed.		
\end{minipage}
\end{table}

==> 15 Minutes-4/tables/ivregs_access_usage_with_controls.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jul 25, 2022 - 10:34:05 PM
\begin{table}[!htbp] \centering 
  \caption{OLS and IV estimates of the relationship between 15-minute usage and access across neighborhoods (Census Block Groups) in New York City} 
  \label{tbl: iv access usage}
\resizebox{\textwidth}{!}{\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\toprule
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
 & \multicolumn{4}{c}{Usage (\% of trips within a 15m walk)} \\ 
 & OLS & \multicolumn{3}{c}{IV estimates} \\ \cmidrule(r){2-2} \cmidrule(r){3-5} 
 & (1) & (2) & (3) & (4)\\\midrule
 Access to amenities within a 15m walk & 0.878$^{***}$ & 1.384$^{***}$ & 1.064$^{***}$ & 1.096$^{***}$ \\ 
  & (0.033) & (0.135) & (0.120) & (0.123) \\ 
  & & & & \\ 
 Population Density (Log) & 3.554$^{***}$ &  & 3.319$^{***}$ & 3.283$^{***}$ \\ 
  & (0.254) &  & (0.355) & (0.356) \\ 
  & & & & \\ 
 Median Income (Log) & $-$2.386$^{***}$ &  & $-$2.505$^{***}$ & $-$2.583$^{***}$ \\ 
  & (0.362) &  & (0.467) & (0.479) \\ 
  & & & & \\ 
 \% Pop. with no car & 0.146$^{***}$ &  & 0.133$^{***}$ & 0.138$^{***}$ \\ 
  & (0.011) &  & (0.014) & (0.014) \\ 
  & & & & \\ 
IV: Log Average Commercial FAR in 1961 Resolution &  & \checkmark & \checkmark & \checkmark \\ 
Distance to City Center & \checkmark & \checkmark & \checkmark & \checkmark \\ 
1960 Population and Housing Density & \checkmark & \checkmark & \checkmark & \checkmark \\ 
1960 Workers by Industry & \checkmark & \checkmark & \checkmark & \checkmark \\ 
1960 Poor and Non-white Families &  &  & & \checkmark \\ 
First stage F-stat &  & 133.21 & 150.21 & 135.58 \\ 
Observations & 4,804 & 5,170 & 4,804 & 4,804 \\ 
\bottomrule
% Access within 15-minute walk & 0.367$^{***}$ & 0.729$^{***}$ & 0.570$^{***}$ & 0.597$^{***}$ \\ 
%   & (0.021) & (0.078) & (0.069) & (0.071) \\ 
%   & & & & \\ 
%  Population Density (Log) & 0.267$^{***}$ &  & 0.239$^{***}$ & 0.228$^{***}$ \\ 
%   & (0.018) &  & (0.024) & (0.025) \\ 
%   & & & & \\ 
%  Median Income (Log) & $-$0.204$^{***}$ &  & $-$0.248$^{***}$ & $-$0.254$^{***}$ \\ 
%   & (0.026) &  & (0.034) & (0.035) \\ 
%   & & & & \\ 
%  \% Pop. with no car & 0.010$^{***}$ &  & 0.008$^{***}$ & 0.008$^{***}$ \\ 
%   & (0.001) &  & (0.001) & (0.001) \\ 
% Distance to City Center & \checkmark & \checkmark & \checkmark & \checkmark \\ 
% 1960 Population and Housing Density & \checkmark & \checkmark & \checkmark & \checkmark \\ 
% 1960 Workers by Industry & \checkmark & \checkmark & \checkmark & \checkmark \\ 
% 1960 Poor and Non-white Families &  &  &  & \checkmark \\ 
% First stage F-stat & NA & 369.23 & 392.5 & 394.44 \\ 
% Observations & 4,804 & 5,170 & 4,804 & 4,804 \\ \bottomrule
\end{tabular}} 
	\begin{minipage}{1\linewidth}													\scriptsize \textsl{Notes.---} The table reports OLS and IV estimates of the relationship between 15-minute usage and access for neighborhoods in New York City. Column 1 reports OLS estimates of the relationship between 15-minute usage and access for New York City, controlling for distance to the city center and a host of socio-economic controls for 1960, including population and housing density and the share of workers by industry. Columns 2-4 report the IV estimates. Columns 2 and 3 also control for distance to the city center, population and housing density and the share of workers by industry. Column 4 includes additional controls for the share of poor and non-white families in 1960. The covariates included in these models come from \citet{twinam2017} and \citet{martynov2022}.    
Robust standard errors are in parentheses. The coefficients with *** are significant at the 1\% confidence level; with ** are significant at the 5\% confidence level; and with * are significant at the 10\% confidence level.
	\end{minipage}	
\end{table} 



==> 15 Minutes-4/tables/regs_far_usage_access.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jul 25, 2022 - 10:34:05 PM
\begin{table}[!htbp] \centering 
  \caption{First-stage and reduced-form estimates of 1961 zoning regulation on current access and usage.} 
    \label{regs_far_usage_access}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{\extracolsep{5pt}}lcccc} \toprule
 & \multicolumn{4}{c}{\textsl{Dependent variable:}} \\ 
 & \multicolumn{2}{c}{Access} & \multicolumn{2}{c}{Usage (\% trips)} \\\cmidrule(r){2-3}\cmidrule(r){4-5}
 & (1) & (2) & (3) & (4)\\ 
\midrule 
 Log Average Commercial FAR & 0.927$^{***}$ & 0.548$^{***}$ & 7.185$^{***}$ & 5.872$^{***}$ \\ 
  & (0.026) & (0.029) & (0.607) & (0.710) \\ 
  & & & & \\ 
Controls: &  &  &  &  \\ 
Distance to City Center &  & \checkmark &  & \checkmark \\ 
1960 Population and Housing Density &  & \checkmark &  & \checkmark \\ 
1960 Workers by Industry & & \checkmark & & \checkmark \\ 
Observations & 5,170 & 5,170 & 5,170 & 5,170 \\ 
\bottomrule
\end{tabular} 
} 
	\begin{minipage}{1\linewidth}													\scriptsize \textsl{Notes.---} The table reports first-stage (columns 1 and 2) and reduced-form (columns 3 and 4) estimates of the relationship between 1961 zoning and access and usage for neighborhoods in New York City. Columns 2 and 4 control for distance to the city center and a host of socio-economic controls for 1960, including population and housing density and the share of workers by industry.  The covariates included in these models come from \citet{twinam2017} and \citet{martynov2022}.  Robust standard errors are in parentheses. The coefficients with *** are significant at the 1\% confidence level; with ** are significant at the 5\% confidence level; and with * are significant at the 10\% confidence level.
	\end{minipage}	
\end{table} 

==> 15 Minutes-4/tables/regs_usage_residual_cbg_city.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, May 31, 2022 - 12:46:15 AM
\begin{table}[!ht] \centering 
  \caption{Relationship between 15-minute usage and access across neighborhoods (Census Block Groups) and Urban areas} 
 \label{tbl: main covariates}
\resizebox{\textwidth}{!}{\begin{tabular}{@{\extracolsep{5pt}}lcccccccc} 
\toprule
 & \multicolumn{8}{c}{\textsl{Dependent Variable:} 15-minute Usage (\% of trips)} \\
 & \multicolumn{4}{c}{Across Neighborhoods} & \multicolumn{4}{c}{Across Urban Areas} \\ \cmidrule(r){2-5} \cmidrule(r){6-9}
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ \midrule
 15-minute Access & 0.761$^{***}$ & 0.696$^{***}$ & 0.686$^{***}$ & 0.693$^{***}$ & 0.604$^{***}$ & 0.481$^{***}$ & 0.426$^{***}$ & 0.424$^{***}$ \\ 
  & (0.006) & (0.007) & (0.007) & (0.007) & (0.015) & (0.035) & (0.031) & (0.031) \\ 
  & & & & & & & & \\ 
 Pop Density Log &  & 0.787$^{***}$ & 0.225 & 0.473$^{***}$ &  & 2.473$^{***}$ & 2.308$^{***}$ & 2.471$^{***}$ \\ 
  &  & (0.265) & (0.174) & (0.165) &  & (0.634) & (0.564) & (0.576) \\ 
  & & & & & & & & \\ 
 Median Income Log &  & $-$4.282$^{***}$ & $-$1.954$^{***}$ & $-$1.583$^{***}$ &  & $-$2.989$^{***}$ & $-$0.171 & $-$0.340 \\ 
  &  & (0.239) & (0.210) & (0.231) &  & (0.703) & (0.680) & (0.704) \\ 
  & & & & & & & & \\ 
 \% Education: BA + &  & 0.008 & $-$0.016$^{***}$ & $-$0.012$^{***}$ &  & 0.050$^{***}$ & 0.034$^{***}$ & 0.029$^{**}$ \\ 
  &  & (0.005) & (0.004) & (0.004) &  & (0.014) & (0.012) & (0.013) \\ 
  & & & & & & & & \\ 
 \% White &  & $-$0.007 & 0.008 & 0.006 &  & $-$0.002 & 0.017$^{*}$ & 0.014 \\ 
  &  & (0.005) & (0.005) & (0.005) &  & (0.010) & (0.009) & (0.009) \\ 
  & & & & & & & & \\ 
 \% No-car Households &  &  & 0.175$^{***}$ & 0.176$^{***}$ &  &  & 0.483$^{***}$ & 0.464$^{***}$ \\ 
  &  &  & (0.009) & (0.009) &  &  & (0.046) & (0.051) \\ 
  & & & & & & & & \\ 
 Transit Density Log &  &  &  & 6.323$^{**}$ &  &  &  & $-$1.651 \\ 
  &  &  &  & (2.934) &  &  &  & (6.352) \\ 
  & & & & & & & & \\ 
 Average Commute (mi) &  &  &  & 0.209$^{***}$ &  &  &  & $-$0.018 \\ 
  &  &  &  & (0.013) &  &  &  & (0.011) \\ 
  & & & & & & & & \\ 
Urban Area FE & \checkmark & \checkmark & \checkmark & \checkmark &  &  &  &  \\ 
Observations & 147,760 & 143,417 & 143,417 & 143,401 & 418 & 418 & 418 & 418 \\ 
R$^{2}$ & 0.736 & 0.752 & 0.759 & 0.761 & 0.806 & 0.819 & 0.857 & 0.858 \\ 
\bottomrule
\end{tabular}} 
\begin{minipage}{1\linewidth}
\scriptsize \textsl{Notes.---} The table reports OLS estimates of the relationship between 15-minute usage and access.
Columns 1 to 4 report estimates at the neighborhood level (controlling for urban area fixed effects) and columns 5 to 8 report estimates at the urban area level. The covariates included in columns 2 to 4 and 6 to 8 come from the American Community Survey and the \emph{National Transit Map} from the Bureau of Transportation Statistics.    
Robust standard errors clustered at the county level are in parentheses. The coefficients with *** are significant at the 1\% confidence level; with ** are significant at the 5\% confidence level; and with * are significant at the 10\% confidence level.					
\end{minipage}

\end{table} 



==> 15 Minutes-4/tables/table_segregation.tex <==
% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, May 31, 2022 - 12:46:15 AM
\begin{table}[!htbp] \centering 
  \caption{Relationship between experienced segregation and local trips for neighborhoods of different income levels.} 
  \label{tbl : psi usage income} 
\resizebox{\textwidth}{!}{\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\toprule
&\multicolumn{4}{c}{\textit{Dependent variable:}} \\ &\multicolumn{4}{c}{Physical Segregation Index (PSI)} \\ 
& \multicolumn{2}{c}{Main 15 urban areas} & \multicolumn{2}{c}{Full sample} \\ \cmidrule(r){2-3}\cmidrule(r){4-5}
 & (1) & (2) & (3) & (4)\\\midrule
Usage $\times$ Low income &       0.165$^{***}$&                    &       0.070$^{***}$&                    \\
            &     (0.029)        &                    &     (0.013)        &                    \\
Usage $\times$ Moderate-low income &       0.024        &                    &      -0.002        &                    \\
            &     (0.015)        &                    &     (0.007)        &                    \\
Usage $\times$ Moderate-high income &      -0.081$^{***}$&                    &      -0.064$^{***}$&                    \\
            &     (0.017)        &                    &     (0.007)        &                    \\
Usage $\times$ High income &      -0.113$^{***}$&                    &      -0.064$^{***}$&                    \\
            &     (0.022)        &                    &     (0.010)        &                    \\
Access $\times$ Low income &                    &       0.182$^{***}$&                    &       0.039$^{***}$\\
            &                    &     (0.041)        &                    &     (0.014)        \\
Access $\times$ Moderate-low income &                    &       0.024$^{*}$  &                    &      -0.019$^{***}$\\
            &                    &     (0.014)        &                    &     (0.006)        \\
Access $\times$ Moderate-high income &                    &      -0.096$^{***}$&                    &      -0.076$^{***}$\\
            &                    &     (0.014)        &                    &     (0.007)        \\
Access $\times$ High income &                    &      -0.119$^{***}$&                    &      -0.071$^{***}$\\
            &                    &     (0.015)        &                    &     (0.010)        \\
\\ Urban area fixed effects & \checkmark & \checkmark & \checkmark & \checkmark \\ R-squared&        0.26        &        0.28        &        0.34        &        0.35        \\
Observations&       34594        &       34594        &      143411        &      143411        \\
\bottomrule
\end{tabular}} 

\begin{minipage}{1\linewidth}
	\scriptsize \textsl{Notes.---} The table reports OLS estimates of the relationship between experienced segregation and 15-minute usage (columns 1 and 3) and access (columns 2 and 4). We provide estimates for neighborhoods in the select sample of cities from Panel C of Figure \ref{fig: usage map} and for all neighborhoods in our sample. The table reports estimates interacted with dummies for low income neighborhoods (bottom quartile of income in urban area), moderate-low income neighborhoods (second quartile),  moderate-high income neighborhoods (third quartile), and high income neighborhoods (top quartile).   
Robust standard errors clustering at the urban area level are in parentheses. The coefficients with *** are significant at the 1\% confidence level; with ** are significant at the 5\% confidence level; and with * are significant at the 10\% confidence level.
\end{minipage}
\label{a6}
\end{table} 

==> 15 Minutes-4/tables/usage_index_correlation_table.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sun, Oct 23, 2022 - 14:13:38
% Requires LaTeX packages: dcolumn 
\begin{table}[H] \centering 
  \caption{Correlation of various measures of local living with 15 min. usage} 
  \label{tbl:corr cut-offs} 
\resizebox{\textwidth}{!}{\begin{tabular}{L{3cm}cccc}\toprule
\multicolumn{1}{c}{Alternate measure} & \multicolumn{1}{c}{Neighborhood  level correlation} & \multicolumn{1}{c}{Neighborhood level mean} & \multicolumn{1}{c}{Urban area level correlation} & \multicolumn{1}{c}{Urban area level mean} \\ 
& (1) & (2) & (3) & (4) \\\midrule
\multicolumn{1}{c}{15 min. usage} & 1    & 0.225 & 1 & 0.134 \\ 
\multicolumn{1}{c}{10 min. usage} & 0.901 & 0.172 & 0.957 & 0.106 \\ 
\multicolumn{1}{c}{20 min. usage} & 0.941 & 0.282 & 0.982 & 0.188 \\ 
\multicolumn{1}{c}{25 min. usage} & 0.892 & 0.335 & 0.962 & 0.233 \\ 
\multicolumn{1}{c}{Med. trip dist. (km)} & -0.727 & 2.704 & -0.626 & 3.499 \\ 
\multicolumn{1}{c}{Observations} & 147,760 & 147,760 & 418 & 418 \\ \bottomrule
\end{tabular} }
\begin{minipage}{1\linewidth}
\scriptsize \textsl{Notes.---} The table shows neighborhood level correlations and means for different measures of local usage. Column 1 provides the correlation between our main usage measure and alternative measures defined by the share of trips within 10, 20, and 25 minutes, as well as the median trip length. Column 2 reports (unweighted) means for these alternative variables. Columns 3 and 4 aggregate the data to urban areas and report urban area-level correlations and (unweighted) means.
\end{minipage}

\end{table} 

